MEFLUT: Unsupervised 1D Lookup Tables for Multi-exposure Image Fusion

In this paper, we introduce a new approach for high-quality multi-exposure image fusion (MEF). We show that the fusion weights of an exposure can be encoded into a 1D lookup table (LUT), which takes pixel intensity value as input and produces fusion weight as output. We learn one 1D LUT for each exposure, then all the pixels from different exposures can query 1D LUT of that exposure independently for high-quality and efficient fusion. Specifically, to learn these 1D LUTs, we involve attention mechanism in various dimensions including frame, channel and spatial ones into the MEF task so as to bring us significant quality improvement over the state-of-the-art (SOTA). In addition, we collect a new MEF dataset consisting of 960 samples, 155 of which are manually tuned by professionals as ground-truth for evaluation. Our network is trained by this dataset in an unsupervised manner. Extensive experiments are conducted to demonstrate the effectiveness of all the newly proposed components, and results show that our approach outperforms the SOTA in our and another representative dataset SICE, both qualitatively and quantitatively. Moreover, our 1D LUT approach takes less than 4ms to run a 4K image on a PC GPU. Given its high quality, efficiency and robustness, our method has been shipped into millions of Android mobiles across multiple brands world-wide. Code is available at: https://github.com/Hedlen/MEFLUT.

==> include/fig-datasample2.tex <==
\begin{figure*}[h]
\begin{minipage}{1.0\linewidth}
\centerline{\includegraphics[width=\textwidth]{Figs/sample_exp_sub1_1_1.pdf}}
\centerline{\includegraphics[width=\textwidth]{Figs/sample_exp_sub2_1_1.pdf}}
\centerline{\includegraphics[width=\textwidth]{Figs/sample_exp_sub3_1_1.pdf}}
% \vspace{-0.37cm}
% \centerline{Image}
\end{minipage}
\caption{Sample source image sequences with different exposure levels in our dataset. We listed some scenes of (a) Sunny, (b) Cloudy, (c) Night. All data is collected by mobile phones.}
\label{fig:sample_exp2}
\end{figure*}


==> include/fig-disa.tex <==
\begin{figure}[t]
\centering
\includegraphics[trim= 0 246 1320 0,clip,width=0.98\linewidth]{./Figs/disa.pdf}\vspace{-2mm}
\caption{Dilated inception with spatial attention (DISA).}\label{fig:samd_module}\vspace{-2mm}
\end{figure}


==> include/fig-fca.tex <==
\begin{figure}[t!]
\centering
\includegraphics[trim= 0 210 1280 0,clip,width=0.98\linewidth]{./Figs/fca_v2.pdf}\vspace{-2mm}
\caption{Convolution with frame and channel attention (CFCA).}\label{fig:fca_module}\vspace{-2mm}
\end{figure}


==> include/fig-lut.tex <==
\begin{figure*}[htbp]
\centering
\includegraphics[trim=0 240 610 0,clip,width=0.95\linewidth]{./Figs/lutGEN_v3.pdf}\vspace{-2mm}
\caption{Lookup Table (LUT) generation. For each grayscale $v$, we feed the network with a group of LDR images with constant color $v$ and set the LUT matrix by the predicted results as Eq.~\ref{eq:lut-fill}.}\label{fig:pipeline}\vspace{-3mm}
\end{figure*}


==> include/fig-noise.tex <==
\begin{figure}[t]

\centering
% \vspace{-1mm}
\includegraphics[width=1.0\linewidth]{./Figs/noise.pdf}
\vspace{-5mm}
\caption{Our method works together with an image denoise approach. \textbf{Left}: inputs images with noise; \textbf{Middle}: our result without denoise; \textbf{Right}: our result with denoise.}
\vspace{-3mm}
\label{fig:noise}
\end{figure}

==> include/fig-oursvis-su1.tex <==
 \begin{figure*}[t]
   \centering
   \includegraphics[width=1.0\linewidth]{./Figs/ours_vis_su3_2_s.pdf}
   \caption{
  Qualitative comparison of the proposed method with (b) Mertens09~\cite{mertens2009exposure}, (c) Li13~\cite{li2013image}, (d) DeepFuse~\cite{ram2017deepfuse}, (e) MEFNet~\cite{ma2019deep}, (f) IFCNN~\cite{zhang2020ifcnn} and (g) TransMEF~\cite{qu2022transmef} on our test set. Input sequences with different exposures are shown in (a). The Zoomed red box region of the result shows that (h) our method hallucinate more reasonable details in saturated regions. Although (c) Li13 achieves considerable detail in saturated regions, unnatural artifacts appear.
%   Qualitative comparison on our test set. The Zoomed red box region of the result show that (h) our method hallucinate more reasonable details in saturated regions.
   } \label{fig:our_vis_su1}\vspace{-3mm}
 \end{figure*} 

==> include/fig-oursvis2.tex <==
 \begin{figure*}[t]
   \centering
   \includegraphics[width=1.0\linewidth]{./Figs/ours_vis3.pdf}\vspace{-3mm}
   \caption{
  Qualitative comparison of the proposed method with (b) Mertens09~\cite{mertens2009exposure}, (c) Li13~\cite{li2013image}, (d) GGIF~\cite{kou2017multi}, (e) Li20~\cite{li2020fast}, (f) DeepFuse~\cite{ram2017deepfuse}, and (g) MEFNet~\cite{ma2019deep} on our test set. Input sequences with different exposures are shown in (a). The Zoomed red box region of the result shows that (h) our method hallucinate more reasonable details in saturated regions.
%   Qualitative comparison on our test set. The Zoomed red box region of the result show that (h) our method hallucinate more reasonable details in saturated regions.
   } \label{fig:our_vis4}
 \end{figure*} 

==> include/fig-oursvis3.tex <==
 \begin{figure*}[t]
   \centering
   \includegraphics[width=1.0\linewidth]{./Figs/ours_vis_su3_3_s.pdf}
   \caption{
  Qualitative comparison of the proposed method with (b) Mertens09~\cite{mertens2009exposure}, (c) Li13~\cite{li2013image}, (d) Li20~\cite{li2020fast}, (e) DeepFuse~\cite{ram2017deepfuse}, (f) MEFNet~\cite{ma2019deep} and (g) TransMEF~\cite{qu2022transmef} on our test set. Input sequences with different exposures are shown in (a). The Zoomed red box region of the result shows that (h) our method hallucinates more reasonable details in saturated regions. Although (c) Li13 achieves considerable detail in saturated regions, unnatural gray artifacts appear.
%   Qualitative comparison on our test set. The Zoomed red box region of the result show that (h) our method hallucinate more reasonable details in saturated regions.
   } \label{fig:our_vis4}
 \end{figure*} 

==> include/fig-phones.tex <==
 \begin{figure}[ht]
   \centering
   \includegraphics[width=1.0\linewidth]{./Figs/fig3_small.pdf}
   \caption{Qualitative comparison of the proposed method with other method in the existing smartphones, our method hallucinates more reasonable details in saturated regions.
   } \label{fig:our_rebuttal}
   \vspace{-3mm}
 \end{figure} 

==> include/fig-sice_vis2.tex <==
\begin{figure*}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{./Figs/sice_vis_su_1_s.pdf}
% \includegraphics[width=1.0\linewidth]{./Figs/sice_new2.pdf}
\caption{
Qualitative comparison of the proposed method with (c) Mertens09~\cite{mertens2009exposure}, (e) Li13~\cite{li2013image}, (g) DeepFuse~\cite{ram2017deepfuse}, (i) MEFNet~\cite{ma2019deep}, (d) IFCNN~\cite{zhang2020ifcnn} and (f) TransMEF~\cite{qu2022transmef} on SICE~\cite{cai2018learning} dataset. Input sequences with different exposures are shown in (a) and (b). The zoom-in region of the red box shows that (h) our method contributes to a more natural image of the grasses with faithful details. Although (e) Li13 and (g) DeepFuse achieves considerable detail in saturated regions, (e) Li13 has unnatural artifacts, and (g) DeepFuse does not recover enough detail in dark area.
% Qualitative comparison on test set of SICE~\cite{cai2018learning}. The Zoomed red box region of the result show that (h) our method produces a more natural appearance with faithful detail and color reproduction.
} \label{fig:sice_vis2}
\end{figure*}


==> include/fig-time-lut.tex <==
\begin{figure}[t]
\vspace{-2mm}
\centering
\begin{minipage}[t]{0.5\textwidth}
\centering
\includegraphics[width=1.0\linewidth]{./Figs/time_n8.pdf}\vspace{-3mm}
\caption{Running time in milliseconds (ms) on different spatial resolutions ($K=2$).}\label{fig:time}
\end{minipage}
% \hspace{-2mm}
\vspace{-6mm}
\begin{minipage}[t]{0.5\textwidth}
\centering
\includegraphics[width=1.0\linewidth]{./Figs/1d_lut4.pdf}\vspace{-3mm}
\caption{The visualization of the 1D LUTs ($K=3$).}\label{fig:lut_vis}
\end{minipage}
% \vspace{-2mm}
\end{figure}

==> include/tab-Crossover.tex <==
\begin{table}[t]
    \centering
    
    \setlength{\tabcolsep}{8.0 pt}
    \resizebox*{0.98\linewidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
             \multirow{2}*{Metrics}& \multicolumn{5}{c}{Exposure Number ($K$)}   \\ \cline{2-6}
             & 2 & 3 & 4 & 5 & 6 \\ \hline
    PSNR$\uparrow$     & 31.016   & \textbf{31.387} & 31.253    & 30.858   & 30.525   \\ 
    SSIM$\uparrow$     & 0.9528   & \textbf{0.9590}      & 0.9532    & 0.9473    & 0.9432   \\ 
    Q$_\emph{C}$ $\uparrow$  & 0.6024 & \textbf{0.6075} & 0.6013 & 0.5981 & 0.5874\\ 
    MEF-SSIM$\uparrow$ & 0.9669   & \textbf{0.9688}     & 0.9686    & 0.9683     & 0.9656  \\
    \bottomrule
    \end{tabular}}
    \vspace{1mm}
    \caption{Robustness experiment based on three 1D LUTs and the arbitrary number of exposure inputs. The best results being highlighted in bold.}
    \label{table:mutil_frame_test}
    \vspace{-3mm}
\end{table}


==> include/tab-modelArchitecture.tex <==
\begin{table}[t]
%   \vspace{-1mm}
	\centering
% 	\vspace{2mm}
	\setlength{\tabcolsep}{8 pt}
	\resizebox*{0.90\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
CFCA         & DISA         & PSNR$\uparrow$            & SSIM$\uparrow$  & Q$_C$$\uparrow$  & MEF-SSIM$\uparrow$\\ 
           \hline
             &              & 29.648          & 0.9373   &$0.5617$    & 0.9442\\
$\checkmark$ &              & 30.570          & 0.9431   &$0.5943$  & 0.9522\\
             & $\checkmark$ & 30.782          & 0.9482   & $0.5960$  & 0.9598\\
$\checkmark$ & $\checkmark$ & \textbf{31.387} & \textbf{0.9590} & $ \textbf{0.6075}$ & \textbf{0.9688} \\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{Ablation study of the proposed CFCA and DISA modules ($K=3$). }
\label{table:mod}
\vspace{-5mm}

\end{table}


==> include/tab-multi-frames-time-5.tex <==
\begin{table*}[t]
\vspace{-5mm}
\centering
\resizebox{0.88\linewidth}{!}{
\begin{tabular}{
>{\centering\arraybackslash}p{2.5cm}
>{\centering\arraybackslash}p{1.7cm}
>{\centering\arraybackslash}p{4.2cm}
>{\centering\arraybackslash}p{4.2cm}
>{\centering\arraybackslash}p{4.2cm}}
\toprule
                     &\multirow{2}*{Methods}& \multicolumn{3}{c}{Exposure Number ($K$)} \\
                     \cline{3-5}
                     & & 2 & 3 & 4                 \\ \hline
\multirow{7}{*}{CPU} & Mertens09 & 2574.70                        & 3569.85                        & 4623.87                        \\ \cline{2-5}
                     & Li13      & 14335.62                       & 17708.18                       & 20478.79                       \\ \cline{2-5}
                     & GGIF      & 5605.31                        & 8268.27                        & 10860.62                       \\ \cline{2-5}
                     & Li20      & 4056.95                        & 5972.75                        & 7834.62                        \\ \cline{2-5}
                     & DeepFuse  & 6990.85                       & -                                 & -                              \\ \cline{2-5}
					 %& DeepFuse~\cite{ram2017deepfuse} ($*$)  & \textcolor{blue}{6820.85} & - & -                    \\ \cline{2-5}
                     & MEFNet    & \textcolor{blue}{487.53}  (14833.32)                       & \textcolor{blue}{496.63}  (15234.68)                   & \textcolor{blue}{514.95} (15721.16)                       \\ \cline{2-5}
                     %& MEFNet~\cite{ma2019deep} ($*$)    & 14833.32 & \textcolor{blue}{15234.68} & \textcolor{blue}{15721.16} \\ \cline{2-5}
					 & Ours      & \textcolor{red}{439.45}  (54.32)      &\textcolor{red}{452.76} (55.36)                        & \textcolor{red}{484.64} (56.17)                        \\ \hline
					 %& Ours ($*$)      & \textcolor{red}{54.23} & \textcolor{red}{55.36} & \textcolor{red}{56.17} \\ \hline
\multirow{3}{*}{GPU}  & DeepFuse  & \textcolor{blue}{4.08}                       & -                              & -                              \\ \cline{2-5}
          & MEFNet    & 7.21  (5.48) & \textcolor{blue}{7.65} (5.71)
          & \textcolor{blue}{7.72} (6.23) \\
          \cline{2-5}
         %& MEFNet~\cite{ma2019deep} ($*$)    & 7.21 & \textcolor{blue}{7.65} & \textcolor{blue}{7.72} \\ \cline{2-5}
		 & Ours      & \textcolor{red}{3.06} (0.53)  & \textcolor{red}{3.54} (0.56) & \textcolor{red}{3.89} (0.61) \\ \hline
%& Ours ($*$)      & \textcolor{red}{3.06} & \textcolor{red}{3.54} & \textcolor{red}{3.89}         \
\multirow{2}{*}{Qualcomm}  & DeepFuse  & \textcolor{blue}{400}                       & -                              & -                   \\ \cline{2-5}
%& DeepFuse~\cite{ram2017deepfuse} ($*$)  & \textcolor{blue}{4.08}                          & -                              & -                              \\ \cline{2-5}
          & MEFNet    & 600  (530) & \textcolor{blue}{700} (580) & \textcolor{blue}{890} (623) \\
          \cline{2-5}
         %& MEFNet~\cite{ma2019deep} ($*$)    & 7.21 & \textcolor{blue}{7.65} & \textcolor{blue}{7.72} \\ \cline{2-5}
\multirow{1}{*}{SM8250}		 & Ours      & \textcolor{red}{150} (53)  & \textcolor{red}{254} (56) & \textcolor{red}{324} (61) \\
%& Ours ($*$)      & \textcolor{red}{3.06} & \textcolor{red}{3.54} & \textcolor{red}{3.89}         \\

\bottomrule
\end{tabular}}
\vspace{-3mm}
\caption{Running time of MEF methods on image sequence of $2048^2$ resolution, on different $K$ settings in milliseconds (ms). The best and 2nd best are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively. `-' means not supported by DeepFuse~\cite{ram2017deepfuse} for such a test. For values in `()', they are calculated by disabling GFU, so that the speed of LUT only can be directly measured.}
\label{table:diff_frame_time}
\vspace{-4mm}
\end{table*}




==> include/tab-multi-time-new.tex <==

\begin{table}[t]
%   \vspace{-1mm}
	\centering
% 	\vspace{-7mm}
	\setlength{\tabcolsep}{6 pt}
\resizebox{0.96\linewidth}{!}{
\begin{tabular}{
>{\centering\arraybackslash}p{1.0cm}
>{\centering\arraybackslash}p{1.3cm}
>{\centering\arraybackslash}p{1.7cm}
>{\centering\arraybackslash}p{1.7cm}
>{\centering\arraybackslash}p{1.7cm}
}
\toprule
                     &\multirow{2}*{Methods}& \multicolumn{3}{c}{Exposure Number ($K$)} \\
                     \cline{3-5}
                     & & 2 & 3 & 4                 \\ \hline
\multirow{9}{*}{CPU} & Mertens09 & 2575                       & 3570                    & 4624                        \\% \cline{2-5}
                     & Li13       & 14336                       & 17708                      & 20479                      \\% \cline{2-5}
                     & GGIF      & 5605                        & 8268                       & 10861                       \\% \cline{2-5}
                     & Li20      & 4057                        & 5973                        & 7835                        \\% \cline{2-5}
                     & DeepFuse  & 6991                        & -                                 & -                              \\% \cline{2-5}
                     & MEFNet    & \textcolor{blue}{522}(14833)                        & \textcolor{blue}{531}(15097)                     & \textcolor{blue}{550}(15641)                        \\% \cline{2-5}
                      & IFCNN    & 12901                        & 18123                     & 23954                        \\%
                       & TransMEF    & 344168                        & -                     & -                        \\%
                     & Ours      & \textcolor{red}{439}(54)       &\textcolor{red}{453}(56)                          & \textcolor{red}{485}(60)                        \\ \hline
\multirow{5}{*}{GPU}  & DeepFuse  & \textcolor{blue}{5.08}                          & -                              & -                              \\% \cline{2-5}
          & MEFNet    & 7.21(5.48) & \textcolor{blue}{7.65}(5.92) & \textcolor{blue}{7.72}(6.31) \\ %\cline{2-5}
           & IFCNN    & 307 & 360 & 417 \\ %\cline{2-5}
           & TransMEF    & 11524 & - & - \\ %\cline{2-5}
         & Ours      & \textcolor{red}{3.06}(0.53) & \textcolor{red}{3.54}(0.61) & \textcolor{red}{3.89}(0.65) \\
         \hline
\multirow{1}{*}{M-CPU} 
         & Ours      & 11.78 & 12.75 & 13.32 \\
\bottomrule
% \multicolumn{5}{c}{(a) Running time in various exposure numbers with GFU enabled.}\vspace{1mm}
\end{tabular}}
% \resizebox{0.92\linewidth}{!}{
% \begin{tabular}{
% >{\centering\arraybackslash}p{3.5cm}
% >{\centering\arraybackslash}p{2.5cm}
% >{\centering\arraybackslash}p{2.5cm}
% }
% \toprule
% Methods  & CPU     & GPU   \\ %\hline
% MEFNet   & 14833.32 &5.48       \\ %\hline
% Ours     & \textcolor{red}{54.23}   & \textcolor{red}{0.53}   \\
% \bottomrule
% \multicolumn{3}{c}{(b) Running time in 2 exposures with GFU disabled.}
% \end{tabular}}
% \vspace{-1mm}
\caption{Running time of MEF methods on different $K$ settings in milliseconds (ms). `-' means not supported by DeepFuse and TransMEF for such a test. For values in `()', we only compare our method with MEFNet, they are calculated by disabling GFU so that the speed of LUT only can be directly measured. M-CPU denotes the mobile CPU. The best and 2nd best are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}\vspace{-3mm}
\label{table:diff_frame_time}
\end{table}

==> include/tab-multi-time-new2.tex <==

\begin{table}[t]
%   \vspace{-1mm}
	\centering
% 	\vspace{-7mm}
	\setlength{\tabcolsep}{6 pt}
\resizebox{0.96\linewidth}{!}{
\begin{tabular}{
>{\centering\arraybackslash}p{1.0cm}
>{\centering\arraybackslash}p{1.3cm}
>{\centering\arraybackslash}p{1.7cm}
>{\centering\arraybackslash}p{1.7cm}
>{\centering\arraybackslash}p{1.7cm}
}
\toprule
                     &\multirow{2}*{Methods}& \multicolumn{3}{c}{Exposure Number ($K$)} \\
                     \cline{3-5}
                     & & 2 & 3 & 4                 \\ \hline
\multirow{9}{*}{CPU} & Mertens09 & 2575                       & 3570                    & 4624                        \\% \cline{2-5}
                     & Li13       & 14336                       & 17708                      & 20479                      \\% \cline{2-5}
                     & GGIF      & 5605                        & 8268                       & 10861                       \\% \cline{2-5}
                     & Li20      & 4057                        & 5973                        & 7835                        \\% \cline{2-5}
                     & DeepFuse  & 6991                        & -                                 & -                              \\% \cline{2-5}
                     & MEFNet    & \textcolor{blue}{622}(14833)                        & \textcolor{blue}{631}(15097)                     & \textcolor{blue}{650}(15641)                        \\% \cline{2-5}
                      & IFCNN    & 12901                        & 18123                     & 23954                        \\%
                       & TransMEF    & 344168                        & -                     & -                        \\%
                     & Ours      & \textcolor{red}{239}(54)       &\textcolor{red}{253}(56)                          & \textcolor{red}{285}(60)                        \\ \hline
\multirow{5}{*}{GPU}  & DeepFuse  & \textcolor{blue}{6.28}                          & -                              & -                              \\% \cline{2-5}
          & MEFNet    & 7.21(5.48) & \textcolor{blue}{7.65}(5.92) & \textcolor{blue}{7.72}(6.31) \\ %\cline{2-5}
           & IFCNN    & 307 & 360 & 417 \\ %\cline{2-5}
           & TransMEF    & 11524 & - & - \\ %\cline{2-5}
         & Ours      & \textcolor{red}{2.14}(0.53) & \textcolor{red}{2.37}(2.61) & \textcolor{red}{1.89}(0.65) \\
         \hline
\multirow{1}{*}{M-CPU} 
         & Ours      & 11.78 & 12.75 & 13.32 \\
\bottomrule
% \multicolumn{5}{c}{(a) Running time in various exposure numbers with GFU enabled.}\vspace{1mm}
\end{tabular}}
% \resizebox{0.92\linewidth}{!}{
% \begin{tabular}{
% >{\centering\arraybackslash}p{3.5cm}
% >{\centering\arraybackslash}p{2.5cm}
% >{\centering\arraybackslash}p{2.5cm}
% }
% \toprule
% Methods  & CPU     & GPU   \\ %\hline
% MEFNet   & 14833.32 &5.48       \\ %\hline
% Ours     & \textcolor{red}{54.23}   & \textcolor{red}{0.53}   \\
% \bottomrule
% \multicolumn{3}{c}{(b) Running time in 2 exposures with GFU disabled.}
% \end{tabular}}
% \vspace{-1mm}
\caption{Running time of MEF methods on different $K$ settings in milliseconds (ms). `-' means not supported by DeepFuse and TransMEF for such a test. For values in `()', we only compare our method with MEFNet, they are calculated by disabling GFU so that the speed of LUT only can be directly measured. M-CPU denotes the mobile CPU. The best and 2nd best are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}\vspace{-3mm}
\label{table:diff_frame_time}
\end{table}

==> include/tab-multi-times.tex <==
% % \begin{table}[t]
% % \vspace{-7mm}
% % \centering
% % \resizebox{0.92\linewidth}{!}{
% % \begin{tabular}{
% % >{\centering\arraybackslash}p{1.3cm}
% % >{\centering\arraybackslash}p{2.2cm}
% % >{\centering\arraybackslash}p{1.4cm}
% % >{\centering\arraybackslash}p{1.4cm}
% % >{\centering\arraybackslash}p{1.4cm}
% % }
% % \toprule
% %                      &\multirow{2}*{Methods}& \multicolumn{3}{c}{Exposure Number ($K$)} \\
% %                      \cline{3-5}
% %                      & & 2 & 3 & 4                 \\ \hline
% % \multirow{7}{*}{CPU} & Mertens09 & 2574.70                        & 3569.85                        & 4623.87                        \\ \cline{2-5}
% %                      & Li13       & 14335.62                       & 17708.18                       & 20478.79                       \\ \cline{2-5}
% %                      & GGIF      & 5605.31                        & 8268.27                        & 10860.62                       \\ \cline{2-5}
% %                      & Li20      & 4056.95                        & 5972.75                        & 7834.62                        \\ \cline{2-5}
% %                      & DeepFuse  & 6990.85                        & -                                 & -                              \\ \cline{2-5}
% %                      & MEFNet    & \textcolor{blue}{521.53}                        & \textcolor{blue}{530.83}                     & \textcolor{blue}{549.95}                        \\ \cline{2-5}
% %                      & Ours      & \textcolor{red}{439.45}       &\textcolor{red}{452.76}                         & \textcolor{red}{484.64}                         \\ \hline
% % \multirow{3}{*}{GPU}  & DeepFuse  & \textcolor{blue}{5.08}                          & -                              & -                              \\ \cline{2-5}
% %           & MEFNet    & 7.21 & \textcolor{blue}7.65 & \textcolor{blue}7.72 \\ \cline{2-5}
% %          & Ours      & \textcolor{red}{3.06} & \textcolor{red}{3.54} & \textcolor{red}{3.89} \\
% %          \hline
% % \multirow{1}{*}{M-CPU} 
% %          & Ours      & \textcolor{red}{11.78} & \textcolor{red}{12.75} & \textcolor{red}{13.32} \\
% % \bottomrule
% % \multicolumn{5}{c}{(a) Running time in various exposure numbers with GFU enabled.}\vspace{1mm}
% % \end{tabular}}
% % \resizebox{0.92\linewidth}{!}{
% % \begin{tabular}{
% % >{\centering\arraybackslash}p{3.5cm}
% % >{\centering\arraybackslash}p{2.5cm}
% % >{\centering\arraybackslash}p{2.5cm}
% % }
% % \toprule
% % Methods  & CPU     & GPU   \\ \hline
% % MEFNet   & 14833.32 &5.48       \\ \hline
% % Ours     & \textcolor{red}{54.23}   & \textcolor{red}{0.53}   \\
% % \bottomrule
% % \multicolumn{3}{c}{(b) Running time in 2 exposures with GFU disabled.}
% % \end{tabular}}
% % \vspace{-3mm}
% % \caption{Running time of MEF methods on image sequence of 2048s resolution, on different $K$s with GFU enabled (a) and on $K=2$ with GFU disabled (b), in milliseconds (ms). For GFU disabled, we only compare our method with another comparison method MEFNet with GFU, so that the speed of LUT only can be directly measured. `-' means not supported by DeepFuse for such a test. M-CPU denotes the mobile CPU. The best and 2nd best are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively. }\vspace{-6mm}
% % \label{table:diff_frame_time}
% % \end{table}

% \begin{table}[t]
% \vspace{-7mm}
% \centering
% \resizebox{0.98\linewidth}{!}{
% \begin{tabular}{
% >{\centering\arraybackslash}p{0.8cm}
% >{\centering\arraybackslash}p{1.2cm}
% >{\centering\arraybackslash}p{2.2cm}
% >{\centering\arraybackslash}p{2.2cm}
% >{\centering\arraybackslash}p{2.2cm}
% }
% \toprule
%                      &\multirow{2}*{Methods}& \multicolumn{3}{c}{Exposure Number ($K$)} \\
%                      \cline{3-5}
%                      & & 2 & 3 & 4                 \\ \hline
% \multirow{7}{*}{CPU} & Mertens09 & 2574.70                        & 3569.85                        & 4623.87                        \\% \cline{2-5}
%                      & Li13       & 14335.62                       & 17708.18                       & 20478.79                       \\% \cline{2-5}
%                      & GGIF      & 5605.31                        & 8268.27                        & 10860.62                       \\% \cline{2-5}
%                      & Li20      & 4056.95                        & 5972.75                        & 7834.62                        \\% \cline{2-5}
%                      & DeepFuse  & 6990.85                        & -                                 & -                              \\% \cline{2-5}
%                      & MEFNet    & \textcolor{blue}{521.53}(14833.32)                        & \textcolor{blue}{530.83}(15096.81)                     & \textcolor{blue}{549.95}(15640.58)                        \\% \cline{2-5}
%                      & Ours      & \textcolor{red}{439.45}(54.23)       &\textcolor{red}{452.76}(55.87)                          & \textcolor{red}{484.64}(59.80)                        \\ \hline
% \multirow{3}{*}{GPU}  & DeepFuse  & \textcolor{blue}{5.08}                          & -                              & -                              \\% \cline{2-5}
%           & MEFNet    & 7.21(5.48) & \textcolor{blue}7.65(5.92) & \textcolor{blue}7.72(6.31) \\ %\cline{2-5}
%          & Ours      & \textcolor{red}{3.06}(0.53) & \textcolor{red}{3.54}(0.61) & \textcolor{red}{3.89}(0.65) \\
%          \hline
% \multirow{1}{*}{M-CPU} 
%          & Ours      & 11.78 & 12.75 & 13.32 \\
% \bottomrule
% % \multicolumn{5}{c}{(a) Running time in various exposure numbers with GFU enabled.}\vspace{1mm}
% \end{tabular}}
% % \resizebox{0.92\linewidth}{!}{
% % \begin{tabular}{
% % >{\centering\arraybackslash}p{3.5cm}
% % >{\centering\arraybackslash}p{2.5cm}
% % >{\centering\arraybackslash}p{2.5cm}
% % }
% % \toprule
% % Methods  & CPU     & GPU   \\ %\hline
% % MEFNet   & 14833.32 &5.48       \\ %\hline
% % Ours     & \textcolor{red}{54.23}   & \textcolor{red}{0.53}   \\
% % \bottomrule
% % \multicolumn{3}{c}{(b) Running time in 2 exposures with GFU disabled.}
% % \end{tabular}}
% \vspace{-3mm}
% \caption{Running time of MEF methods on image sequence of $2048^2$ resolution, on different $K$ settings in milliseconds (ms). `-' means not supported by DeepFuse for such a test. For values in `()', we only compare our method with another comparison method MEFNet with GFU, they are calculated by disabling GFU, so that the speed of LUT only can be directly measured. M-CPU denotes the mobile CPU. The best and 2nd best are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}\vspace{-5mm}
% \label{table:diff_frame_time}
% \end{table}


% \begin{table}[t]
% \vspace{-7mm}
% \centering
% \resizebox{0.92\linewidth}{!}{
% \begin{tabular}{
% >{\centering\arraybackslash}p{1.3cm}
% >{\centering\arraybackslash}p{2.2cm}
% >{\centering\arraybackslash}p{1.4cm}
% >{\centering\arraybackslash}p{1.4cm}
% >{\centering\arraybackslash}p{1.4cm}
% }
% \toprule
%                      &\multirow{2}*{Methods}& \multicolumn{3}{c}{Exposure Number ($K$)} \\
%                      \cline{3-5}
%                      & & 2 & 3 & 4                 \\ \hline
% \multirow{7}{*}{CPU} & Mertens09 & 2574.70                        & 3569.85                        & 4623.87                        \\ \cline{2-5}
%                      & Li13       & 14335.62                       & 17708.18                       & 20478.79                       \\ \cline{2-5}
%                      & GGIF      & 5605.31                        & 8268.27                        & 10860.62                       \\ \cline{2-5}
%                      & Li20      & 4056.95                        & 5972.75                        & 7834.62                        \\ \cline{2-5}
%                      & DeepFuse  & 6990.85                        & -                                 & -                              \\ \cline{2-5}
%                      & MEFNet    & \textcolor{blue}{521.53}                        & \textcolor{blue}{530.83}                     & \textcolor{blue}{549.95}                        \\ \cline{2-5}
%                      & Ours      & \textcolor{red}{439.45}       &\textcolor{red}{452.76}                         & \textcolor{red}{484.64}                         \\ \hline
% \multirow{3}{*}{GPU}  & DeepFuse  & \textcolor{blue}{5.08}                          & -                              & -                              \\ \cline{2-5}
%           & MEFNet    & 7.21 & \textcolor{blue}7.65 & \textcolor{blue}7.72 \\ \cline{2-5}
%          & Ours      & \textcolor{red}{3.06} & \textcolor{red}{3.54} & \textcolor{red}{3.89} \\
%          \hline
% \multirow{1}{*}{M-CPU} 
%          & Ours      & \textcolor{red}{11.78} & \textcolor{red}{12.75} & \textcolor{red}{13.32} \\
% \bottomrule
% \multicolumn{5}{c}{(a) Running time in various exposure numbers with GFU enabled.}\vspace{1mm}
% \end{tabular}}
% \resizebox{0.92\linewidth}{!}{
% \begin{tabular}{
% >{\centering\arraybackslash}p{3.5cm}
% >{\centering\arraybackslash}p{2.5cm}
% >{\centering\arraybackslash}p{2.5cm}
% }
% \toprule
% Methods  & CPU     & GPU   \\ \hline
% MEFNet   & 14833.32 &5.48       \\ \hline
% Ours     & \textcolor{red}{54.23}   & \textcolor{red}{0.53}   \\
% \bottomrule
% \multicolumn{3}{c}{(b) Running time in 2 exposures with GFU disabled.}
% \end{tabular}}
% \vspace{-3mm}
% \caption{Running time of MEF methods on image sequence of 2048s resolution, on different $K$s with GFU enabled (a) and on $K=2$ with GFU disabled (b), in milliseconds (ms). For GFU disabled, we only compare our method with another comparison method MEFNet with GFU, so that the speed of LUT only can be directly measured. `-' means not supported by DeepFuse for such a test. M-CPU denotes the mobile CPU. The best and 2nd best are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively. }\vspace{-6mm}
% \label{table:diff_frame_time}
% \end{table}

% \begin{table}[t]
% \vspace{-7mm}
% \centering
% \resizebox{0.96\linewidth}{!}{
% \begin{tabular}{
% >{\centering\arraybackslash}p{0.8cm}
% >{\centering\arraybackslash}p{1.1cm}
% >{\centering\arraybackslash}p{2.2cm}
% >{\centering\arraybackslash}p{2.2cm}
% >{\centering\arraybackslash}p{2.2cm}
% }
% \toprule
%                      &\multirow{2}*{Methods}& \multicolumn{3}{c}{Exposure Number ($K$)} \\
%                      \cline{3-5}
%                      & & 2 & 3 & 4                 \\ \hline
% \multirow{7}{*}{CPU} & Mertens09 & 2574.70                        & 3569.85                        & 4623.87                        \\% \cline{2-5}
%                      & Li13       & 14335.62                       & 17708.18                       & 20478.79                       \\% \cline{2-5}
%                      & GGIF      & 5605.31                        & 8268.27                        & 10860.62                       \\% \cline{2-5}
%                      & Li20      & 4056.95                        & 5972.75                        & 7834.62                        \\% \cline{2-5}
%                      & DeepFuse  & 6990.85                        & -                                 & -                              \\% \cline{2-5}
%                      & MEFNet    & \textcolor{blue}{521.53}(14833.32)                        & \textcolor{blue}{530.83}(15096.81)                     & \textcolor{blue}{549.95}(15640.58)                        \\% \cline{2-5}
%                      & Ours      & \textcolor{red}{439.45}(54.23)       &\textcolor{red}{452.76}(55.87)                          & \textcolor{red}{484.64}(59.80)                        \\ \hline
% \multirow{3}{*}{GPU}  & DeepFuse  & \textcolor{blue}{5.08}                          & -                              & -                              \\% \cline{2-5}
%           & MEFNet    & 7.21(5.48) & \textcolor{blue}{7.65}(5.92) & \textcolor{blue}{7.72}(6.31) \\ %\cline{2-5}
%          & Ours      & \textcolor{red}{3.06}(0.53) & \textcolor{red}{3.54}(0.61) & \textcolor{red}{3.89}(0.65) \\
%          \hline
% \multirow{1}{*}{M-CPU} 
%          & Ours      & 11.78 & 12.75 & 13.32 \\
% \bottomrule
% % \multicolumn{5}{c}{(a) Running time in various exposure numbers with GFU enabled.}\vspace{1mm}
% \end{tabular}}
% % \resizebox{0.92\linewidth}{!}{
% % \begin{tabular}{
% % >{\centering\arraybackslash}p{3.5cm}
% % >{\centering\arraybackslash}p{2.5cm}
% % >{\centering\arraybackslash}p{2.5cm}
% % }
% % \toprule
% % Methods  & CPU     & GPU   \\ %\hline
% % MEFNet   & 14833.32 &5.48       \\ %\hline
% % Ours     & \textcolor{red}{54.23}   & \textcolor{red}{0.53}   \\
% % \bottomrule
% % \multicolumn{3}{c}{(b) Running time in 2 exposures with GFU disabled.}
% % \end{tabular}}
% \vspace{-3mm}
% \caption{Running time of MEF methods on different $K$ settings in milliseconds (ms). `-' means not supported by DeepFuse for such a test. For values in `()', we only compare our method with MEFNet with GFU, they are calculated by disabling GFU, so that the speed of LUT only can be directly measured. M-CPU denotes the mobile CPU. The best and 2nd best are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}\vspace{-7mm}
% \label{table:diff_frame_time}
% \end{table}


\begin{table}[t]
\vspace{-5mm}
\centering
\resizebox{0.90\linewidth}{!}{
\begin{tabular}{
>{\centering\arraybackslash}p{1.0cm}
>{\centering\arraybackslash}p{1.3cm}
>{\centering\arraybackslash}p{1.7cm}
>{\centering\arraybackslash}p{1.7cm}
>{\centering\arraybackslash}p{1.7cm}
}
\toprule
                     &\multirow{2}*{Methods}& \multicolumn{3}{c}{Exposure Number ($K$)} \\
                     \cline{3-5}
                     & & 2 & 3 & 4                 \\ \hline
\multirow{7}{*}{CPU} & Mertens09 & 2575                       & 3570                    & 4624                        \\% \cline{2-5}
                     & Li13       & 14336                       & 17708                      & 20479                      \\% \cline{2-5}
                     & GGIF      & 5605                        & 8268                       & 10861                       \\% \cline{2-5}
                     & Li20      & 4057                        & 5973                        & 7835                        \\% \cline{2-5}
                     & DeepFuse  & 6991                        & -                                 & -                              \\% \cline{2-5}
                     & MEFNet    & \textcolor{blue}{522}(14833)                        & \textcolor{blue}{531}(15097)                     & \textcolor{blue}{550}(15641)                        \\% \cline{2-5}
                     & Ours      & \textcolor{red}{439}(54)       &\textcolor{red}{453}(56)                          & \textcolor{red}{485}(60)                        \\ \hline
\multirow{3}{*}{GPU}  & DeepFuse  & \textcolor{blue}{5.08}                          & -                              & -                              \\% \cline{2-5}
          & MEFNet    & 7.21(5.48) & \textcolor{blue}{7.65}(5.92) & \textcolor{blue}{7.72}(6.31) \\ %\cline{2-5}
         & Ours      & \textcolor{red}{3.06}(0.53) & \textcolor{red}{3.54}(0.61) & \textcolor{red}{3.89}(0.65) \\
         \hline
\multirow{1}{*}{M-CPU} 
         & Ours      & 11.78 & 12.75 & 13.32 \\
\bottomrule
% \multicolumn{5}{c}{(a) Running time in various exposure numbers with GFU enabled.}\vspace{1mm}
\end{tabular}}
% \resizebox{0.92\linewidth}{!}{
% \begin{tabular}{
% >{\centering\arraybackslash}p{3.5cm}
% >{\centering\arraybackslash}p{2.5cm}
% >{\centering\arraybackslash}p{2.5cm}
% }
% \toprule
% Methods  & CPU     & GPU   \\ %\hline
% MEFNet   & 14833.32 &5.48       \\ %\hline
% Ours     & \textcolor{red}{54.23}   & \textcolor{red}{0.53}   \\
% \bottomrule
% \multicolumn{3}{c}{(b) Running time in 2 exposures with GFU disabled.}
% \end{tabular}}
\vspace{-3mm}
\caption{Running time of MEF methods on different $K$ settings in milliseconds (ms). `-' means not supported by DeepFuse for such a test. For values in `()', we only compare our method with MEFNet, they are calculated by disabling GFU, so that the speed of LUT only can be directly measured. M-CPU denotes the mobile CPU. The best and 2nd best are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}\vspace{-3mm}
\label{table:diff_frame_time}
\end{table}


==> include/tab-mutilbranchs.tex <==

\begin{table}[t]
  \centering
  \resizebox{0.98\linewidth}{!}{
  \setlength{\tabcolsep}{9 pt}
  \vspace{-3mm}
  \begin{tabular}{c|cccc}
    \toprule %添加表格头部粗线
    Number of Branches & 2 & 3 & 4 & 5\\
    \hline
     PSNR$\uparrow$ & 30.117 & \textbf{31.387} & 30.016 & 28.633\\
     SSIM$\uparrow$ & 0.9570 & \textbf{0.9590} & 0.9578 & 0.9565\\
     Q$_C$ $\uparrow$ & 0.5913& \textbf{0.6075} & 0.5983 & 0.5927\\
     MEF-SSIM$\uparrow$ & 0.9682 & \textbf{0.9688} & 0.9681 & 0.9662\\
    \bottomrule
    Resolution & 32 & 64 & 128 & 256 \\
    \hline
     PSNR$\uparrow$ &  30.421  &30.569 & \textbf{31.387} & 31.383\\
     SSIM$\uparrow$ & 0.9560 & 0.9576 & \textbf{0.9590} & 0.9589\\
     Q$_C$ $\uparrow$ & 0.5989 & 0.6034 & \textbf{0.6075} & 0.6037 \\
     MEF-SSIM$\uparrow$ & 0.9667 & 0.9684 & \textbf{0.9688} & 0.9687\\
    \bottomrule
  \end{tabular}}
  % \vspace{-2mm}
  \caption{The impact of the number of branches of DISA, and the resolution of the down-sampled inputs. The exposure number is set to $K = 3$. The best results being highlighted in bold.}
  \label{table:mo_br}
  \vspace{-4mm}
\end{table}

==> include/tab-noise.tex <==
\begin{table}[t]
   \small
    \centering
    \setlength{\tabcolsep}{6 pt}
    % \vspace{-2mm}
    
    \resizebox{0.90\columnwidth}{!}{
    \begin{tabular}{c|cccc}
    \toprule
    %     & PSNR$\uparrow$  & SSIM$\uparrow$ & \emph{Q}$_\emph{C}$ $\uparrow$ \\
    % \hline
    %     Mertens09 [8] & 31.547    & 0.8851 & 0.3412  \\
    %     Li13 [11]      & 20.133  & 0.8450 & 0.3250 \\
    %     GGIF [13]      & 32.491  & 0.9254 & 0.3361 \\
    %     Li20 [15]      & 28.238  & 0.8528 & 0.3317\\
    %     DeepFuse~\cite{ram2017deepfuse_short}  & 21.221  & 0.7291 & 0.3139 \\
    %     MEFNet [5]   &  \color{blue}32.973&  \color{blue}0.9680 & \color{blue}0.4683 \\
    %     Ours      & \color{red}33.092  & \color{red}0.9704 & \color{red}0.4742\\
        Methods & PSNR &  SSIM & Q$_\emph{C}$ & MEF-SSIM \\\hline
        % &Mertens09~\cite{mertens2009exposure} &  Li13~\cite{li2013image}   &GGIF~\cite{kou2017multi} & Li20~\cite{li2020fast} &DeepFuse~\cite{ram2017deepfuse} &MEFNet~\cite{ma2019deep} & Ours \\
        % \hline
        % PSNR  & 27.981 & 20.043 & 29.451 & 26.320 & 20.122 & \color{blue}29.970 & \color{red}31.590  \\
        % SSIM &0.8515 & 0.8484 & 0.9093 & 0.8101 & 0.6562 & \color{blue}0.9604 & \color{red}0.9624 \\
        % Q$_\emph{C}$  & 0.3412 & 0.3250 & 0.3361 & 0.3317 & 0.3139 & \color{blue}0.4683 & \color{red}0.4742 \\
        % MEF-SSIM & 0.9126 & 0.8855 & 0.9472 & 0.9637 & 0.6892 & \color{blue}0.9637 & \color{red}0.9672 \\
        Mertens09 & 27.981 & 0.8515 & 0.3412 & 0.9126 \\
        Li13 & 20.043 & 0.8484 & 0.3250 & 0.8855 \\
        GGIF & 29.451&0.9093 &0.3361 &0.9472 \\
        Li20 & 26.320&0.8101&0.3317 &0.9637 \\
        DeepFuse &20.122 &0.6562 &0.3139 &0.6892 \\
        MEFNet &\color{blue}29.970 &\color{blue}0.9604 &0.4583 &\color{blue}0.9637 \\
        Ours &\color{red}31.590 &\color{red}0.9624 &\color{blue}0.4683 &\color{red}0.9672 \\
    \bottomrule
\end{tabular}}
\vspace{-2mm}
\caption{We quantitatively compare the performance of existing MEF methods when facing noisy inputs on our night dataset. The exposure number is set to $K=3$. Since DeepFuse~\cite{ram2017deepfuse} takes 2 exposures only, we try several under- and over-exposed combinations, and choose the fused image that achieves the best performance for comparison. The best and 2nd best results are highlighted in {\color{red}red} and in {\color{blue}blue}, respectively. As seen, Ours beats the others in all metrics, achieving robustness under noises.}
    % \vspace{-2mm}
\label{table:noise_input_compare}
\vspace{-4mm}

\end{table}

==> include/tab-res-ourdata.tex <==

% \begin{table*}[t]
%     \label{tab:psnr_noniid}
%     \begin{center}
%     % \vspace{-2mm}
%     \resizebox{0.92\linewidth}{!}{
%     \begin{tabular}{
%     >{\centering\arraybackslash}p{1.9cm}
%     >{\centering\arraybackslash}p{1.9cm}
%     >{\centering\arraybackslash}p{2.2cm}
%     >{\centering\arraybackslash}p{1.5cm}
%     >{\centering\arraybackslash}p{1.5cm}
%     >{\centering\arraybackslash}p{1.5cm}
%     >{\centering\arraybackslash}p{2.0cm}
%     >{\centering\arraybackslash}p{2.0cm}
%     >{\centering\arraybackslash}p{1.5cm}
%     }
%          \toprule
%         Exposure &\multirow{2}*{Metrics} & \multicolumn{7}{c}{Methods} \\
%         \cline{3-9}
%         Number ($K$) & &  Mertens09 &  Li13   &GGIF & Li20 & DeepFuse & MEFNet & Ours \\
%         %& & \cite{mertens2009exposure} & ~\cite{li2013image}  &~\cite{kou2017multi}&~\cite{li2020fast}  &~\cite{ram2017deepfuse} &~\cite{ma2019deep}& \\
%         \hline
%         \multirow{4}*{2} & PSNR$\uparrow$
%                     & 26.886 & 19.475 & 27.172  & 25.997  &23.087 & \textcolor{blue}{29.285}    & \textcolor{red}{29.443}\\
%         %\cline{2-9}
%           &  SSIM$\uparrow$  & 0.8347 &0.8326   &0.9153  &0.8765  &0.7558     & \textcolor{blue}{0.9568}   & \textcolor{red}{0.9587} \\
%         %\cline{2-9}
%           & Q$_\emph{C}$ $\uparrow$  & 0.5531 &0.5166 & 0.5330 & 0.5245 &0.4603     & \textcolor{blue}{0.6796}    & \textcolor{red}{0.6860}\\
%          %\cline{2-9}
%           &  MEF-SSIM$\uparrow$  & 0.9410 &0.8797 &0.9638 & 0.9273 &0.7407     & \textcolor{blue}{0.9733}    & \textcolor{red}{0.9773}\\
%         \hline
%         \multirow{4}*{3} & PSNR$\uparrow$
%                     & 27.328 & 20.922  & 29.437 & 25.396 & -  &   \textcolor{blue}{30.293} & \textcolor{red}{31.387}\\
%         %\cline{2-9}
%           &  SSIM$\uparrow$  &0.8927 &0.8468   &0.9208  &0.8603  &  -        & \textcolor{blue}{0.9569}   &\textcolor{red}{0.9590} \\
%         %\cline{2-9}
%           &  Q$_\emph{C}$ $\uparrow$  & 0.4779 &0.4562 &0.4735  & 0.4742 &  -      &\textcolor{blue}{0.6054}   & \textcolor{red}{0.6075}\\
%         %\cline{2-9}
%           &  MEF-SSIM$\uparrow$  & 0.9452 &0.8955 &0.9592  & 0.9387 &  -      &\textcolor{blue}{0.9670}   & \textcolor{red}{0.9688}\\
%         \hline
%         \multirow{4}*{4} & PSNR$\uparrow$
%                     & 26.154 & 20.471   &27.782  &24.602  & - & \textcolor{blue}{30.072}    & \textcolor{red}{31.025}\\
%         %\cline{2-9}
%         &  SSIM$\uparrow$    & 0.8834 &0.8276   &0.9087  &0.8448  & -      & \textcolor{blue}{0.9531}   & \textcolor{red}{0.9548}\\
%         %\cline{2-9}
%         &  Q$_\emph{C}$ $\uparrow$    & 0.4379 & 0.4107   &0.4359  & 0.4371 & -     & \textcolor{blue}{0.05493}     &  \textcolor{red}{0.5571}\\

%         %\cline{2-9}
%         &  MEF-SSIM$\uparrow$    & 0.9360 &0.8897   &0.9528  & 0.9096 & -     & \textcolor{blue}{0.9588}     &  \textcolor{red}{0.9603}\\
%         \bottomrule
%         \multicolumn{9}{c}{(a) Results on our dataset.}
%     \end{tabular}}\\%\vspace{1.0mm}
%     \resizebox{0.92\linewidth}{!}{
%     \begin{tabular}{
% 	    >{\centering\arraybackslash}p{1.9cm}
%     >{\centering\arraybackslash}p{1.9cm}
%     >{\centering\arraybackslash}p{2.2cm}
%     >{\centering\arraybackslash}p{1.5cm}
%     >{\centering\arraybackslash}p{1.5cm}
%     >{\centering\arraybackslash}p{1.5cm}
%     >{\centering\arraybackslash}p{2.0cm}
%     >{\centering\arraybackslash}p{2.0cm}
%     >{\centering\arraybackslash}p{1.5cm}}
%         \toprule
%         Exposure &\multirow{2}*{Metrics} & \multicolumn{7}{c}{Methods} \\
%         \cline{3-9}
%         Number ($K$) & &  Mertens09 &  Li13   &GGIF & Li20 &DeepFuse &MEFNet & Ours \\
%         %& & \cite{mertens2009exposure} & ~\cite{li2013image}  &~\cite{kou2017multi}&~\cite{li2020fast}  &~\cite{ram2017deepfuse} &~\cite{ma2019deep}& \\
%         \hline
%         \multirow{4}*{2} & PSNR$\uparrow$
%                     & 21.531 & 19.380   & 21.316 &21.072 &  20.915 & \textcolor{blue}{21.483}    & \textcolor{red}{21.894}\\
%         %\cline{2-9}
%           &  SSIM$\uparrow$  & 0.7833 &0.7732   &0.7929  &0.7743  &0.6872     & \textcolor{blue}{0.7963}   & \textcolor{red}{0.8067} \\
%         %\cline{2-9}
%           & Q$_\emph{C}$ $\uparrow$  & 0.7759 &0.7056  &0.7709 & 0.7747 &0.6406     & \textcolor{blue}{0.7721}   & \textcolor{red}{0.7934}\\
%         %\cline{2-9}
%           &  MEF-SSIM$\uparrow$  & 0.9589 &0.9451  &0.9692 & 0.9498 &0.8590     & \textcolor{blue}{0.9743}   & \textcolor{red}{0.9845}\\

%         \bottomrule
%         \multicolumn{9}{c}{(b) Results on SICE~\cite{cai2018learning} dataset.}
%     \end{tabular}}

%     \end{center}
%     \vspace{-5mm}
%     \caption{The PSNR, SSIM, Q$_\emph{C}$, MEF-SSIM of all methods on our test set (a) and SICE dataset (b). We quantitatively compare the performance of existing MEF methods with ours on various exposure numbers $K$ in (a), while keeping SICE's settings, i.e. $K=2$ in (b). The best and 2nd best results are highlighted in \textcolor{red}{red} and in \textcolor{blue}{blue}, respectively. As seen, ours beats the others in all settings and both datasets.`-' means not applicable, as DeepFuse can only takes two images as input.}
%      \label{table:ourd}
%     \vspace{-6mm}
% \end{table*}


\begin{table*}[t]
    \label{tab:psnr_noniid}
    \begin{center}
    % \vspace{-2mm}
    \resizebox{0.98\linewidth}{!}{
    \begin{tabular}{
    >{\centering\arraybackslash}p{1.9cm}
    >{\centering\arraybackslash}p{1.9cm}
    >{\centering\arraybackslash}p{2.2cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{2.0cm}
    >{\centering\arraybackslash}p{2.0cm}
    >{\centering\arraybackslash}p{1.5cm}
    }
         \toprule
        Exposure &\multirow{2}*{Metrics} & \multicolumn{7}{c}{Methods} \\
        \cline{3-9}
        Number ($K$) & &  Mertens09 &  Li13   &GGIF & Li20 & DeepFuse & MEFNet & Ours \\
        %& & \cite{mertens2009exposure} & ~\cite{li2013image}  &~\cite{kou2017multi}&~\cite{li2020fast}  &~\cite{ram2017deepfuse} &~\cite{ma2019deep}& \\
        \hline
        \multirow{4}*{2} & PSNR$\uparrow$
                    & 26.886 & 19.475 & 27.172  & 25.997  &23.087 & \textcolor{blue}{29.285}    & \textcolor{red}{29.443}\\
        %\cline{2-9}
          &  SSIM$\uparrow$  & 0.8347 &0.8326   &0.9153  &0.8765  &0.7558     & \textcolor{blue}{0.9568}   & \textcolor{red}{0.9587} \\
        %\cline{2-9}
          & Q$_\emph{C}$ $\uparrow$  & 0.5531 &0.5166 & 0.5330 & 0.5245 &0.4603     & \textcolor{blue}{0.6796}    & \textcolor{red}{0.6860}\\
         %\cline{2-9}
          &  MEF-SSIM$\uparrow$  & 0.9410 &0.8797 &0.9638 & 0.9273 &0.7407     & \textcolor{blue}{0.9733}    & \textcolor{red}{0.9773}\\
        \hline
        \multirow{4}*{3} & PSNR$\uparrow$
                    & 27.328 & 20.922  & 29.437 & 25.396 & -  &   \textcolor{blue}{30.293} & \textcolor{red}{31.387}\\
        %\cline{2-9}
          &  SSIM$\uparrow$  &0.8927 &0.8468   &0.9208  &0.8603  &  -        & \textcolor{blue}{0.9569}   &\textcolor{red}{0.9590} \\
        %\cline{2-9}
          &  Q$_\emph{C}$ $\uparrow$  & 0.4779 &0.4562 &0.4735  & 0.4742 &  -      &\textcolor{blue}{0.6054}   & \textcolor{red}{0.6075}\\
        %\cline{2-9}
          &  MEF-SSIM$\uparrow$  & 0.9452 &0.8955 &0.9592  & 0.9387 &  -      &\textcolor{blue}{0.9670}   & \textcolor{red}{0.9688}\\
        \hline
        \multirow{4}*{4} & PSNR$\uparrow$
                    & 26.154 & 20.471   &27.782  &24.602  & - & \textcolor{blue}{30.072}    & \textcolor{red}{31.025}\\
        %\cline{2-9}
        &  SSIM$\uparrow$    & 0.8834 &0.8276   &0.9087  &0.8448  & -      & \textcolor{blue}{0.9531}   & \textcolor{red}{0.9548}\\
        %\cline{2-9}
        &  Q$_\emph{C}$ $\uparrow$    & 0.4379 & 0.4107   &0.4359  & 0.4371 & -     & \textcolor{blue}{0.5493}     &  \textcolor{red}{0.5571}\\

        %\cline{2-9}
        &  MEF-SSIM$\uparrow$    & 0.9360 &0.8897   &0.9528  & 0.9096 & -     & \textcolor{blue}{0.9588}     &  \textcolor{red}{0.9603}\\
        \bottomrule
        \multicolumn{9}{c}{(a) Results on our dataset.}
    \end{tabular}}\\%\vspace{1.0mm}
    \resizebox{0.98\linewidth}{!}{
    \begin{tabular}{
	    >{\centering\arraybackslash}p{1.9cm}
    >{\centering\arraybackslash}p{1.9cm}
    >{\centering\arraybackslash}p{2.2cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{2.0cm}
    >{\centering\arraybackslash}p{2.0cm}
    >{\centering\arraybackslash}p{1.5cm}}
        \toprule
        Exposure &\multirow{2}*{Metrics} & \multicolumn{7}{c}{Methods} \\
        \cline{3-9}
        Number ($K$) & &  Mertens09 &  Li13   &GGIF & Li20 &DeepFuse &MEFNet & Ours \\
        %& & \cite{mertens2009exposure} & ~\cite{li2013image}  &~\cite{kou2017multi}&~\cite{li2020fast}  &~\cite{ram2017deepfuse} &~\cite{ma2019deep}& \\
        \hline
        \multirow{4}*{2} & PSNR$\uparrow$
                    & 21.531 & 19.380   & 21.316 &21.072 &  20.915 & \textcolor{blue}{21.583}    & \textcolor{red}{21.894}\\
        %\cline{2-9}
          &  SSIM$\uparrow$  & 0.7833 &0.7732   &0.7929  &0.7743  &0.6872     & \textcolor{blue}{0.7963}   & \textcolor{red}{0.8067} \\
        %\cline{2-9}
          & Q$_\emph{C}$ $\uparrow$  & 0.7759 &0.7056  &0.7709 & 0.7747 &0.6406     & \textcolor{blue}{0.7760}   & \textcolor{red}{0.7934}\\
        %\cline{2-9}
          &  MEF-SSIM$\uparrow$  & 0.9589 &0.9451  &0.9692 & 0.9498 &0.8590     & \textcolor{blue}{0.9743}   & \textcolor{red}{0.9845}\\

        \bottomrule
        \multicolumn{9}{c}{(b) Results on SICE~\cite{cai2018learning} dataset.}
    \end{tabular}}

    \end{center}
    \vspace{-5mm}
    \caption{The PSNR, SSIM, Q$_\emph{C}$, MEF-SSIM of all methods on our test set (a) and SICE dataset (b). The best and 2nd best results are highlighted in \textcolor{red}{red} and in \textcolor{blue}{blue}, respectively. `-' means not applicable, as DeepFuse can only takes two images as input.}
     \label{table:ourd}
    \vspace{-5mm}
\end{table*}


==> include/tab-res-ourdata2.tex <==
\begin{table*}[t]
    \label{tab:psnr_noniid}
    \begin{center}
    % \vspace{-2mm}
    \resizebox{0.98\linewidth}{!}{
    \begin{tabular}{
    >{\centering\arraybackslash}p{1.9cm}
    >{\centering\arraybackslash}p{1.9cm}
    >{\centering\arraybackslash}p{2.2cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{2.0cm}
    >{\centering\arraybackslash}p{2.0cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}
    }
         \toprule
        Exposure &\multirow{2}*{Metrics} & \multicolumn{9}{c}{Methods} \\
        \cline{3-11}
        Number ($K$) & &  Mertens09 &  Li13   &GGIF & Li20 & DeepFuse & MEFNet & IFCNN & TransMEF & Ours \\
        %& & \cite{mertens2009exposure} & ~\cite{li2013image}  &~\cite{kou2017multi}&~\cite{li2020fast}  &~\cite{ram2017deepfuse} &~\cite{ma2019deep}& \\
        \hline
        \multirow{4}*{2} & PSNR$\uparrow$
                    & 26.886 & 19.475 & 27.172  & 25.997  &23.087 & \textcolor{blue}{29.285}  & &  & \textcolor{red}{29.443}\\
        %\cline{2-9}
          &  SSIM$\uparrow$  & 0.8347 &0.8326   &0.9153  &0.8765  &0.7558     & \textcolor{blue}{0.9568}   & \textcolor{red}{0.9587} \\
        %\cline{2-9}
          & Q$_\emph{C}$ $\uparrow$  & 0.5531 &0.5166 & 0.5330 & 0.5245 &0.4603     & \textcolor{blue}{0.6796}    & \textcolor{red}{0.6860}\\
         %\cline{2-9}
          &  MEF-SSIM$\uparrow$  & 0.9410 &0.8797 &0.9638 & 0.9273 &0.7407     & \textcolor{blue}{0.9733}    & \textcolor{red}{0.9773}\\
        \hline
        \multirow{4}*{3} & PSNR$\uparrow$
                    & 27.328 & 20.922  & 29.437 & 25.396 & -  &   \textcolor{blue}{30.293} & \textcolor{red}{31.387}\\
        %\cline{2-9}
          &  SSIM$\uparrow$  &0.8927 &0.8468   &0.9208  &0.8603  &  -        & \textcolor{blue}{0.9569}   &\textcolor{red}{0.9590} \\
        %\cline{2-9}
          &  Q$_\emph{C}$ $\uparrow$  & 0.4779 &0.4562 &0.4735  & 0.4742 &  -      &\textcolor{blue}{0.6054}   & \textcolor{red}{0.6075}\\
        %\cline{2-9}
          &  MEF-SSIM$\uparrow$  & 0.9452 &0.8955 &0.9592  & 0.9387 &  -      &\textcolor{blue}{0.9670}   & \textcolor{red}{0.9688}\\
        \hline
        \multirow{4}*{4} & PSNR$\uparrow$
                    & 26.154 & 20.471   &27.782  &24.602  & - & \textcolor{blue}{30.072}    & \textcolor{red}{31.025}\\
        %\cline{2-9}
        &  SSIM$\uparrow$    & 0.8834 &0.8276   &0.9087  &0.8448  & -      & \textcolor{blue}{0.9531}   & \textcolor{red}{0.9548}\\
        %\cline{2-9}
        &  Q$_\emph{C}$ $\uparrow$    & 0.4379 & 0.4107   &0.4359  & 0.4371 & -     & \textcolor{blue}{0.5493}     &  \textcolor{red}{0.5571}\\

        %\cline{2-9}
        &  MEF-SSIM$\uparrow$    & 0.9360 &0.8897   &0.9528  & 0.9096 & -     & \textcolor{blue}{0.9588}     &  \textcolor{red}{0.9603}\\
        \bottomrule
        \multicolumn{11}{c}{(a) Results on our dataset.}
    \end{tabular}}\\%\vspace{1.0mm}
    \resizebox{0.98\linewidth}{!}{
    \begin{tabular}{
	    >{\centering\arraybackslash}p{1.9cm}
    >{\centering\arraybackslash}p{1.9cm}
    >{\centering\arraybackslash}p{2.2cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{2.0cm}
    >{\centering\arraybackslash}p{2.0cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}
    >{\centering\arraybackslash}p{1.5cm}}
        \toprule
        Exposure &\multirow{2}*{Metrics} & \multicolumn{9}{c}{Methods} \\
        \cline{3-11}
        Number ($K$) & &  Mertens09 &  Li13   &GGIF & Li20 &DeepFuse &MEFNet & IFCNN & TransMEF & Ours \\
        %& & \cite{mertens2009exposure} & ~\cite{li2013image}  &~\cite{kou2017multi}&~\cite{li2020fast}  &~\cite{ram2017deepfuse} &~\cite{ma2019deep}& \\
        \hline
        \multirow{4}*{2} & PSNR$\uparrow$
                    & 21.531 & 19.380   & 21.316 &21.072 &  20.915 & 21.583  &\textcolor{blue}{21.6256} & 21.6012 & \textcolor{red}{21.894}\\
        %\cline{2-9}
          &  SSIM$\uparrow$  & 0.7833 &0.7732   &0.7929  &0.7743  &0.6872     & 0.7763  &0.7839 & \textcolor{blue}{0.7865} & \textcolor{red}{0.8067} \\
        %\cline{2-9}
          & Q$_\emph{C}$ $\uparrow$  & 0.7759 &0.7056  &0.7709 & 0.7747 &0.6406     & 0.7760  & 0.7789&  \textcolor{blue}{0.7837}& \textcolor{red}{0.7934}\\
        %\cline{2-9}
          &  MEF-SSIM$\uparrow$  & 0.9589 &0.9451  &0.9692 & 0.9498 &0.8590     & 0.9743  & 0.9786 &  \textcolor{blue}{0.9802}& \textcolor{red}{0.9845}\\

        \bottomrule
        \multicolumn{11}{c}{(b) Results on SICE~\cite{cai2018learning} dataset.}
    \end{tabular}}

    \end{center}
    \vspace{-5mm}
    \caption{The PSNR, SSIM, Q$_\emph{C}$, MEF-SSIM of all methods on our test set (a) and SICE dataset (b). The best and 2nd best results are highlighted in \textcolor{red}{red} and in \textcolor{blue}{blue}, respectively. `-' means not applicable, as DeepFuse and TransMEF can only takes two images as input.}
     \label{table:ourd}
    \vspace{-3mm}
\end{table*}


==> include/tab-upsampling-noise.tex <==
\begin{table}[t]
  \small
    \centering
    % \setlength{\tabcolsep}{2.0 pt}
    % % \vspace{-2mm}
\resizebox*{0.98\linewidth}{!}{
\setlength{\tabcolsep}{1.5 pt}
  \begin{tabular}{cccccc}
    \toprule %添加表格头部粗线
    Variants & PSNR$\uparrow$  & SSIM$\uparrow$ & Q$_C$$\uparrow$ & MEF-SSIM$\uparrow$ & Running Time (ms)\\
    \hline
    %   PSNR & 31.189 &  \textbf{33.941} \\
    %   SSIM & 0.9648 & \textbf{0.9691} \\
    %   MEF-SSIM & 0.9678 & \textbf{0.9692} \\
    %   Running Time (ms)&  \textbf{1.51} & 3.54 \\
    BU & 29.189 & 0.9548 & $0.6052$& 0.9674 & \textbf{0.95} \\
    GFU & \textbf{31.387} & \textbf{0.9590} &  $\textbf{0.6075}$&\textbf{0.9688} & 3.54 \\
    % w/o. GFU & \textbf{31.387} & \textbf{0.9590} &  $\textbf{0.6075}$&\textbf{0.9688} & 3.54 \\
    \bottomrule
  \end{tabular}}
  % \vspace{-2mm}
 \caption{The effectiveness of GFU, tested under $K=3$. BU denotes the Bilinear upsampling. The best results being highlighted in bold.}
\label{table:diff_up}
\vspace{1mm}
\resizebox{0.98\columnwidth}{!}{
    \setlength{\tabcolsep}{8 pt}
    \begin{tabular}{c|cccc}
    \toprule
    %     & PSNR$\uparrow$  & SSIM$\uparrow$ & \emph{Q}$_\emph{C}$ $\uparrow$ \\
    % \hline
    %     Mertens09 [8] & 31.547    & 0.8851 & 0.3412  \\
    %     Li13 [11]      & 20.133  & 0.8450 & 0.3250 \\
    %     GGIF [13]      & 32.491  & 0.9254 & 0.3361 \\
    %     Li20 [15]      & 28.238  & 0.8528 & 0.3317\\
    %     DeepFuse~\cite{ram2017deepfuse_short}  & 21.221  & 0.7291 & 0.3139 \\
    %     MEFNet [5]   &  \color{blue}32.973&  \color{blue}0.9680 & \color{blue}0.4683 \\
    %     Ours      & \color{red}33.092  & \color{red}0.9704 & \color{red}0.4742\\
        Methods & PSNR$\uparrow$ &  SSIM$\uparrow$ & Q$_\emph{C}$$\uparrow$ & MEF-SSIM$\uparrow$ \\\hline
        % &Mertens09~\cite{mertens2009exposure} &  Li13~\cite{li2013image}   &GGIF~\cite{kou2017multi} & Li20~\cite{li2020fast} &DeepFuse~\cite{ram2017deepfuse} &MEFNet~\cite{ma2019deep} & Ours \\
        % \hline
        % PSNR  & 27.981 & 20.043 & 29.451 & 26.320 & 20.122 & \color{blue}29.970 & \color{red}31.590  \\
        % SSIM &0.8515 & 0.8484 & 0.9093 & 0.8101 & 0.6562 & \color{blue}0.9604 & \color{red}0.9624 \\
        % Q$_\emph{C}$  & 0.3412 & 0.3250 & 0.3361 & 0.3317 & 0.3139 & \color{blue}0.4683 & \color{red}0.4742 \\
        % MEF-SSIM & 0.9126 & 0.8855 & 0.9472 & 0.9637 & 0.6892 & \color{blue}0.9637 & \color{red}0.9672 \\
        Mertens09 & 27.981 & 0.8515 & 0.3412 & 0.9126 \\
        Li13 & 20.043 & 0.8484 & 0.3250 & 0.8855 \\
        GGIF & 29.451&0.9093 &0.3361 &0.9472 \\
        Li20 & 26.320&0.8101&0.3317 &0.9637 \\
        DeepFuse &20.122 &0.6562 &0.3139 &0.6892 \\
        MEFNet &29.631 &0.9567 & 0.4548 & 0.9605 \\
        IFCNN & 29.970 &0.9597 &0.4574 & 0.9622 \\ 
        TransMEF & \color{blue}30.370 &\color{blue}0.9604 &\color{blue}0.4583 &\color{blue}0.9639 \\ 
        Ours &\color{red}31.590 &\color{red}0.9624 &\color{red}0.4683 &\color{red}0.9672 \\
    \bottomrule
\end{tabular}}
% \vspace{-2mm}
\caption{We quantitatively compare the performance of existing MEF methods when facing noisy inputs on our night dataset. The exposure number is set to $K=3$. Since DeepFuse~\cite{ram2017deepfuse} and TransMEF~\cite{qu2022transmef} takes 2 exposures only, we try several under- and over-exposed combinations, and choose the fused image that achieves the best performance for comparison. The best and 2nd best results are highlighted in {\color{red}red} and in {\color{blue}blue}, respectively. As seen, Ours beats the others in all metrics, achieving robustness under noises.}\label{table:noise_input_compare}
\vspace{-3mm}
\end{table}

==> include/tab-upsampling.tex <==
\begin{table}[t]
  \centering

  \setlength{\tabcolsep}{3 pt}
\resizebox*{0.9\linewidth}{!}{
  \begin{tabular}{cccccc}
    \toprule %添加表格头部粗线
    Variants & PSNR  & SSIM & Q$_C$ & MEF-SSIM & Running Time (ms)\\
    \hline
    %   PSNR & 31.189 &  \textbf{33.941} \\
    %   SSIM & 0.9648 & \textbf{0.9691} \\
    %   MEF-SSIM & 0.9678 & \textbf{0.9692} \\
    %   Running Time (ms)&  \textbf{1.51} & 3.54 \\
    BU & 29.189 & 0.9548 & $0.6052$& 0.9674 & \textbf{1.51} \\
    GFU & \textbf{31.387} & \textbf{0.9590} &  $\textbf{0.6075}$&\textbf{0.9688} & 3.54 \\
    % w/o. GFU & \textbf{31.387} & \textbf{0.9590} &  $\textbf{0.6075}$&\textbf{0.9688} & 3.54 \\
    \bottomrule
  \end{tabular}}
  \vspace{-3mm}
 \caption{The effectiveness of GFU, tested under $K=3$. BU denotes the Bilinear Upsampling.}
\label{table:diff_up}
  \vspace{-6mm}
\end{table}


==> include/tab-validity-noise.tex <==
\begin{table}[t]
  \small
    \centering
    % \setlength{\tabcolsep}{2.0 pt}
    % % \vspace{-2mm}
\resizebox{0.96\linewidth}{!}{
  \setlength{\tabcolsep}{4 pt}
  \begin{tabular}{c|cccc}
    \toprule %添加表格头部粗线
    Methods  & PSNR$\uparrow$ & SSIM$\uparrow$ & Q$_C$$\uparrow$ & MEF-SSIM$\uparrow$ \\
    \hline
     MEFNet & 25.315 & 0.8924 & 0.5575 & 0.9064 \\
     Ours & \textbf{31.387} & \textbf{0.9590} & \textbf{0.6075} & \textbf{0.9688} \\
     
    \bottomrule
  \end{tabular}}
  \vspace{-2mm}
  \caption{The Compatibility of the network to 1D LUTs.The exposure number is set to K = 3. The best results being highlighted in bold.}\label{table:validity}
\resizebox{0.98\columnwidth}{!}{
    \setlength{\tabcolsep}{3.5 pt}
    \begin{tabular}{c|cccc}
    \toprule
    %     & PSNR$\uparrow$  & SSIM$\uparrow$ & \emph{Q}$_\emph{C}$ $\uparrow$ \\
    % \hline
    %     Mertens09 [8] & 31.547    & 0.8851 & 0.3412  \\
    %     Li13 [11]      & 20.133  & 0.8450 & 0.3250 \\
    %     GGIF [13]      & 32.491  & 0.9254 & 0.3361 \\
    %     Li20 [15]      & 28.238  & 0.8528 & 0.3317\\
    %     DeepFuse~\cite{ram2017deepfuse_short}  & 21.221  & 0.7291 & 0.3139 \\
    %     MEFNet [5]   &  \color{blue}32.973&  \color{blue}0.9680 & \color{blue}0.4683 \\
    %     Ours      & \color{red}33.092  & \color{red}0.9704 & \color{red}0.4742\\
        Methods & PSNR$\uparrow$ &  SSIM$\uparrow$ & Q$_\emph{C}$$\uparrow$ & MEF-SSIM$\uparrow$ \\\hline
        % &Mertens09~\cite{mertens2009exposure} &  Li13~\cite{li2013image}   &GGIF~\cite{kou2017multi} & Li20~\cite{li2020fast} &DeepFuse~\cite{ram2017deepfuse} &MEFNet~\cite{ma2019deep} & Ours \\
        % \hline
        % PSNR  & 27.981 & 20.043 & 29.451 & 26.320 & 20.122 & \color{blue}29.970 & \color{red}31.590  \\
        % SSIM &0.8515 & 0.8484 & 0.9093 & 0.8101 & 0.6562 & \color{blue}0.9604 & \color{red}0.9624 \\
        % Q$_\emph{C}$  & 0.3412 & 0.3250 & 0.3361 & 0.3317 & 0.3139 & \color{blue}0.4683 & \color{red}0.4742 \\
        % MEF-SSIM & 0.9126 & 0.8855 & 0.9472 & 0.9637 & 0.6892 & \color{blue}0.9637 & \color{red}0.9672 \\
        Mertens09 & 27.981 & 0.8515 & 0.3412 & 0.9126 \\
        Li13 & 20.043 & 0.8484 & 0.3250 & 0.8855 \\
        GGIF & 29.451&0.9093 &0.3361 &0.9472 \\
        Li20 & 26.320&0.8101&0.3317 &0.9637 \\
        DeepFuse &20.122 &0.6562 &0.3139 &0.6892 \\
        MEFNet &\color{blue}29.970 &\color{blue}0.9604 &\color{blue}0.4683 &\color{blue}0.9637 \\
        Ours &\color{red}31.590 &\color{red}0.9624 &\color{blue}0.4683 &\color{red}0.9672 \\
    \bottomrule
\end{tabular}}
\vspace{-2mm}
\caption{We quantitatively compare the performance of existing MEF methods when facing noisy inputs on our night dataset. The exposure number is set to $K=3$. Since DeepFuse~\cite{ram2017deepfuse} takes 2 exposures only, we try several under- and over-exposed combinations, and choose the fused image that achieves the best performance for comparison. The best and 2nd best results are highlighted in {\color{red}red} and in {\color{blue}blue}, respectively. As seen, Ours beats the others in all metrics, achieving robustness under noises.}\label{table:noise_input_compare}

  \vspace{-3mm}
\end{table}

==> include/tab-validity.tex <==

\begin{table}[t]
  \centering
  \resizebox{0.95\linewidth}{!}{
  \setlength{\tabcolsep}{11 pt}
  \begin{tabular}{c|cccc}
    \toprule %添加表格头部粗线
    Methods  & PSNR$\uparrow$ & SSIM$\uparrow$ & Q$_C$$\uparrow$ & MEF-SSIM$\uparrow$ \\
    \hline
     MEFNet & 25.315 & 0.8924 & 0.5575 & 0.9064 \\
     Ours & \textbf{31.387} & \textbf{0.9590} & \textbf{0.6075} & \textbf{0.9688} \\
     
    \bottomrule
  \end{tabular}}
  \vspace{-3mm}
  \caption{The Effectiveness of our network to LUTs ($K=3$).}
  \label{table:validity}
  \vspace{-5mm}
\end{table}


==> rebuttal/include/fig-dark-regions.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.86\linewidth]{./rebuttal/dark_regions2.pdf}\vspace{-4mm}
    \caption{Visual comparison with several state-of-the-art methods in dark regions, as indicated by the red arrow.
  }\vspace{-3mm}
  \label{fig:dark}
\end{figure}

==> rebuttal/include/fig-sice-re.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.94\linewidth]{./rebuttal/sice-iidmef.pdf}\vspace{-3mm}
    \caption{Visual comparison of our method with IID-MEF. 
  }\vspace{-2.5mm}
  \label{fig:sixe-re}
\end{figure}

==> rebuttal/include/tab-align-deghost-time.tex <==
\begin{table}[t]
  \centering
  \resizebox{0.9\linewidth}{!}{
  \setlength{\tabcolsep}{11 pt}
  \begin{tabular}{c|cccc}
    \toprule %添加表格头部粗线
    Methods  & Baseline  & w/ Deghosting &  w/ ECC & w/ (ECC and Deghosting)\\
    \midrule
     Running time ($ms$) & 12.75 & 18.03  & 37.32 & 42.60 \\
    \bottomrule
  \end{tabular}}
  \vspace{-3mm}
  \caption{Running time after adding alignment and deghosting operations, our MEFLUT as the baseline. The running platform is Qualcomm SM8250. The resolution is $2048^2$. ($K=3$).}
  \label{table:align_deghot}
  \vspace{-5.5mm}
\end{table}

==> rebuttal/include/tab-multi-resolution.tex <==
\begin{table}[t]
  \centering
  \resizebox{0.86\linewidth}{!}{
  \setlength{\tabcolsep}{11 pt}
  \begin{tabular}{c|ccccc}
    \toprule %添加表格头部粗线
    Methods  & PSNR$\uparrow$ & SSIM$\uparrow$ & Q$_C$$\uparrow$ & MEF-SSIM$\uparrow$ & Running time (ms) \\
    \hline
     Multi-resolution & \textbf{31.412} & \textbf{0.9621} & \textbf{0.6096} & \textbf{0.9714} & 304.50 \\
     Ours & 31.387 & 0.9590 & 0.6075 & 0.9688 & \textbf{12.75} \\
    \bottomrule
  \end{tabular}}
  \vspace{-3mm}
  \caption{Comparison experiments with the multi-resolution scheme. The running platform is Mobile CPU ($K=3$).}
  \label{table:linear}
  \vspace{-3mm}
\end{table}

==> rebuttal/include/tab-sice-re.tex <==
\begin{table}[t]
  \centering
  \resizebox{0.84\linewidth}{!}{
  \setlength{\tabcolsep}{11 pt}
  \begin{tabular}{c|ccccc}
    \toprule %添加表格头部粗线
    Methods  & PSNR$\uparrow$ & SSIM$\uparrow$ & Q$_C$$\uparrow$ & MEF-SSIM$\uparrow$ & Running time ($ms$) \\
    \midrule
     IID-MEF & 21.639 & 0.7857 & 0.7723 & 0.9634 & 1232.18 \\
     Ours & \textbf{21.894} & \textbf{0.8067} & \textbf{0.7934} & \textbf{0.9845} & \textbf{3.06} \\
    \bottomrule
  \end{tabular}}
  \vspace{-3mm}
  \caption{Quantitative and complexity comparisons with IID-MEF on SICE. The running platform is NVIDIA 2080Ti. ($K=2$).}
  \label{table:sice-re}
  \vspace{-2.5mm}
\end{table}
